Masked Label Prediction: Unified Message Passing Model for Semi-Supervised Classification

Graph neural network (GNN) and label propagation algorithm (LPA) are both message passing algorithms, which have achieved superior performance in semi-supervised classification. GNN performs feature propagation by a neural network to make predictions, while LPA uses label propagation across graph adjacency matrix to get results. However, there is still no effective way to directly combine these two kinds of algorithms. To address this issue, we propose a novel Unified Message Passaging Model (UniMP) that can incorporate feature and label propagation at both training and inference time. First, UniMP adopts a Graph Transformer network, taking feature embedding and label embedding as input information for propagation. Second, to train the network without overfitting in self-loop input label information, UniMP introduces a masked label prediction strategy, in which some percentage of input label information are masked at random, and then predicted. UniMP conceptually unifies feature propagation and label propagation and is empirically powerful. It obtains new state-of-the-art semi-supervised classification results in Open Graph Benchmark (OGB).

==> key_point.tex <==
IJCAI  Important Dates:
Submission site opening: December 30, 2020
Abstract submission deadline: January 13, 2021 (11:59PM UTC-12)
Author information deadline: January 16, 2021 (11:59PM UTC-12)
Full paper submission deadline: January 20, 2021 (11:59PM UTC-12)
Summary reject notification: February 07, 2021
Author response period: March 24-28, 2021
Paper notification: April 30, 2021

=======================================
论文格式修改：
Tabel title 在下方

论文主体修改
0. 统一一下 abstract 和 introduction
1. 增加related work
2. 给 UniMP 图标注  （a)、（b）、（c）, 方便后续Unimp描述
3. Ablation study: 突出消融的两部分：(1) incorporate label and feature (2) graph transformer 的消融实验。
4. ablation 的消融实验和 sota 的一致性问题



1. 删除没利用的citation。
2. Table 名称要直接明了。
3. 语法问题。







========================================
resubmissions 的 材料
Resubmissions: Authors of papers that have been rejected at any peer-reviewed conference within the past 6 months must declare the resubmission by including a cover letter with their submission. The cover letter should summarize the main reasons for rejection and should describe the changes the authors have made to address the reviewers’ comments. The cover letter should be put in a separate file, along with the previous reviews and previous anonymized rejected submission. Such resubmissions must contain, in a single PDF file (different from the IJCAI-21 paper file):

the cover letter, starting with the title of the rejected paper, the tracking number (if any), and the name of the conference to which this paper was submitted,
the full reviews from the rejected conference,
the anonymized version of the rejected paper.
This resubmission information will be visible to reviewers only during the discussion phase after they submit their initial review.A paper rejected from a peer-reviewed conference within the past 6 months will be rejected without further review if the authors do not declare the resubmission.

To submit resubmission file PDF, first upload your submission. You will then be able to upload resubmission file from the author console as a supplementary file. There are two entries for supplementary files: one is “TechnicalAppendix”, which is the normal supplementary file for the main paper; and the other one is “ResubmissionFile”, to which you should upload the resubmission file. Note that the maximal size of the resubmission PDF is 10M.





